Spikformer: When Spiking Neural Network Meets Transformer

We consider two biologically plausible structures, the Spiking Neural Network (SNN) and the self-attention mechanism. The former offers an energy-efficient and event-driven paradigm for deep learning, while the latter has the ability to capture feature dependencies, enabling Transformer to achieve good performance. It is intuitively promising to explore the marriage between them. In this paper, we consider leveraging both self-attention capability and biological properties of SNNs, and propose a novel Spiking Self Attention (SSA) as well as a powerful framework, named Spiking Transformer (Spikformer). The SSA mechanism in Spikformer models the sparse visual feature by using spike-form Query, Key, and Value without softmax. Since its computation is sparse and avoids multiplication, SSA is efficient and has low computational energy consumption. It is shown that Spikformer with SSA can outperform the state-of-the-art SNNs-like frameworks in image classification on both neuromorphic and static datasets. Spikformer (66.3M parameters) with comparable size to SEW-ResNet-152 (60.2M,69.26%) can achieve 74.81% top1 accuracy on ImageNet using 4 time steps, which is the state-of-the-art in directly trained SNNs models.

==> 07_backup_content.tex <==
% Current position encoding methods [2, 4, 56] mainly focus on the order and the position of input patches and ignore the distance between the patches which is essential for the PMER. That is, we need an appropriate metric to evaluate the relevance of each patch for PMER. Learned Perceptual Image Patch Similarity (LPIPS) metric[23] is mainly used in assessing
% the perceptual similarity between two images, which can measure the distance between the patches in the vision transformer encoder. As shown in figure 4, the distance of semantic similarity between an image patch and two adjacent patches is not the same. That is, relative distance between patches based on LPIPS can be introduced to the TRMER as an  extra supplement of spatial features.

% Due to the transfer invarint and local global spatial modeling capacity, CNN methods has natural advantages to extract the spatial features of images. Though current transformer-based methods have focus on the spatial modeling in 2D images by kinds of position encoding methods, it is still not enough for PMER which contains kinds of spatial relationship: the spatial between math symbols, the spatial relationship between groups of MS, the spatial information of the whole math expression. Based on the above insight, we adopting a dual-branch encoder to process the spatial and text feature separately. A query is divided into two parts according to the number of heads. One of them is fed to a conv-mixer-like module to extract the spatial feature and the other is fead to normal attention module to learn the text recognition. The two feature will be concatenated  before a MLP layer. Such dual-branch mechanism can focus the spatial and text information meanwhile and couple them in the next layer, which has been illustrated to be effective in PMER.(May be should also disscuss the long spatial dependency)
% Based on the above insight, we combine the relative distance between patches with conditional position encoding. This ESM can take into account both the position information of patches and the distance information between patches. The input of ESM is non-overlap patches with~$P \in \mathbb{R}^{N \times C}$~where~$C = H \times W$~is the number of patches.Figure 5 and Equation 5 illustrate how we obtain the LPIPS distance based on the transformer-based backbone. Except for the first layer that uses input features directly, we calculate LPIPS by sampling feature stack from the last three layers of each stage. After  unit-normalizing features in the channel dimension, we compute the~$\ell_2$~distance among patches in the whole feature map and  scale the activations channel-wise by a learning vector~$w^l \in \mathds{R}^{C_l}$.

% As a task that involves both processing image and predicting math symbol sequence, the image features should focus on current sequences and adjust the position information instead of stay the same. However, original transformer decoder updates the feature of predicted sequence when passing through layers when the image feature from encoder without changing. To alleviate above issue, we consider applying an updated relative position encoding~(URPE)~module, which can be aware of the sequence-image attention. By using URPE, math symbol sequence can interact with and influence image features, rather than unilaterally updating themselves. The framework of sequence-position-aware decoder is shown in Figure 6.
